VS-Net: Variable splitting network for accelerated parallel MRI reconstruction

In this work, we propose a deep learning approach for parallel magnetic resonance imaging (MRI) reconstruction, termed a variable splitting network (VS-Net), for an efficient, high-quality reconstruction of undersampled multi-coil MR data. We formulate the generalized parallel compressed sensing reconstruction as an energy minimization problem, for which a variable splitting optimization method is derived. Based on this formulation we propose a novel, end-to-end trainable deep neural network architecture by unrolling the resulting iterative process of such variable splitting scheme. VS-Net is evaluated on complex valued multi-coil knee images for 4-fold and 6-fold acceleration factors. We show that VS-Net outperforms state-of-the-art deep learning reconstruction algorithms, in terms of reconstruction accuracy and perceptual quality. Our code is publicly available at https://github.com/j-duan/VS-Net.

==> sections/AK.tex <==
% !TeX root=../paper.tex
\section{Modelling biventricular anatomy in patients with PH}
\label{sec:method}
\vspace{-1pt}
\begin{wrapfigure}{ro}{0.4\textwidth}
\vspace{-22pt}
\centering
\includegraphics[width=0.4\textwidth]{figure/0.pdf}
\vspace{-20pt}
\caption{Short-axis images of a healthy subject (left) and a PH subject (right), including the anatomical explanation of both LV and RV. The desired epicardial contours (red) and endocardial contours (yellow) from both ventricles are plotted.}
\vspace{-22pt}
\label{fig:HPH}
\end{wrapfigure}
To illustrate cardiac morphology in patients with PH, Fig~\ref{fig:HPH} shows the difference in CMR images from a representative healthy subject and a PH subject. In health, the RV is crescentic in short-axis views and triangular in long-axis views, wrapping around the thicker-walled LV. In PH, the initial hypertrophic response of the RV increases contractility but is followed invariably by progressive dilatation and failure heralding clinical deterioration and ultimately death. During this deterioration, the dilated RV pushes onto the LV to deform and lose its roundness. Moreover, in PH the myocardium around RV become much thicker than a healthy one, allowing PH cardiac morphology to be modelled by a nested level set. Next, we incorporate the biventricular anatomy of PH hearts into our model for automated segmentation of LV and RV cavities and myocardium.


==> sections/results.tex <==
% !TeX root=../paper.tex

\section{Experimental results}
\label{sec:experiments}
\textbf{Data:} Experiments were performed using short-axis CMR images from 430 PH patients. For each patient, 10 to 16 short-axis slices roughly covering the whole heart were acquired. Each short-axis image has resolution of $1.5 \times 1.5 \times 8.0\;\rm{mm}^3$. Due to the large slice thickness of the short-axis slices and the inter-slice shift caused by respiratory motion, we train the FCN in a 2D fashion and apply the DNLS method to segment each slice separately. The ground truth region labels were generated using a semi-automatic process which included a manual correction step by an experienced clinical expert. Region labels for each subject contain the left and right ventricular blood pools and myocardial walls for all 430 subjects at end-diastolic (ED) and end-systolic (ES) frames. The ground truth edge labels are derived from the region label maps by identifying pixels with label transitions. The dataset was randomly split into training (400 subjects) and validation (30 subjects) subsets. For image pre-processing, all training images were reshaped to the same size of $160 \times 160$ with zero-padding, and image intensity was normalised to the range of $[0, 1]$ before training. 

 \textbf{Parameters:} The following parameters were used for the experiments in this work: First, there are six parameters associated with finding a desirable solution to (\ref{eq:transformedFunction}). They are the weighting parameter $\lambda$ (1), regularisation parameter $\epsilon$ (1.5), two levels $c_1$ (0) and $c_2$ (8), time step $t$ (0.1), and iteration number (200). Second, for training the network, we use Adam SGD with learning rate (0.001) and batch size (two subjects) for each of 50000 iterations. The weight $\alpha$ in (\ref{eq:REloss}) is set to 1. We perform data augmentation on-the-fly, which includes random translation, rotation, scaling and intensity rescaling of the input images and labels at each iteration. In this way, the network is made robust against new images as it would have seen millions of different inputs by the end of training. Note that data augmentation is crucial to obtain better results. Training took approx. 10 hours (50000 iterations) on an Nvidia Titan XP GPU, while testing took 5s in order to segment all the images for one subject at ED and ES. 
\begin{figure}[h!] 
\vspace{-10pt}
\centering  
{\includegraphics[width=0.99\textwidth]{figure/compare1.pdf}}\\
\vspace{-5pt}
\caption{Visual comparison of segmentation results from the vanilla CNN, CRF-CNN and proposed method. LV$\&$RV cavities and myocardium are delineated using yellow and red contours. GT stands for ground truth.}
\label{fig:visual}
\vspace{-20pt}
\end{figure}

%\begin{table}[h!]
%\vspace{-20pt}
%\centering
%\caption{Quantitative comparison of segmentation results from the vanilla CNN, CRF-CNN and proposed method, in terms of Dice metric (mean$\pm$standard deviation) and computation time at testing stage.}
%\begin{tabular}{ccccc} \toprule
%{Methods} & {LV\&RV Cavities}     & {Myocardium} & {Time} \\ \midrule
%Vanilla CNN \cite{bai2017human}            & 0.902$\pm$0.047          & 0.703$\pm$0.091           & $\sim$\textbf{0.06}s  \\
%CRF-CNN     \cite{krahenbuhl2011efficient} & 0.911$\pm$0.045          & 0.712$\pm$0.082           & $\sim$2s  \\
%Proposed DNLS                              &\textbf{0.925$\pm$0.032} & \textbf{0.772$\pm$0.058}  & $\sim$5s  \\ \midrule
%\end{tabular}
%\label{tb:numb}
%\vspace{-15pt}
%\end{table}


\begin{table}[h!]
\centering
\caption{Quantitative comparison of segmentation results from the vanilla CNN, CRF-CNN and proposed method, in terms of Dice metric (mean$\pm$standard deviation) and computation time at testing stage.}
\begin{tabular}{ccccc} \toprule
{Methods} & {LV\&RV Cavities}     & {Myocardium} & {Time} \\ \midrule
Vanilla CNN \cite{bai2017human}            & 0.902$\pm$0.047          & 0.703$\pm$0.091           & $\sim$\textbf{0.06}s  \\
CRF-CNN     \cite{krahenbuhl2011efficient} & 0.911$\pm$0.045          & 0.712$\pm$0.082           & $\sim$2s  \\
Proposed DNLS                              &\textbf{0.925$\pm$0.032} & \textbf{0.772$\pm$0.058}  & $\sim$5s  \\ \midrule
\end{tabular}
\label{tb:numb}
\vspace{-15pt}
\end{table}

\textbf{Comparsion:} The segmentation performance was evaluated by computing the Dice overlap metric between the automated and ground truth segmentations for LV $\&$ RV cavities and myocardium. We compared our method with the vanilla CNN proposed in \cite{bai2017human}, the code for which is publicly available. DNLS was also compared with the vanilla CNN with a conditional random field (CRF) \cite{krahenbuhl2011efficient} refinement (CRF-CNN). In Fig~\ref{fig:visual}, visual comparison suggests that DNLS provides significant segmentation improvements over CNN and CRF-CNN. For example, at the base of the right ventricle both CNN and CRF-CNN fail to retain the correct anatomical relationship between endocardium and epicardium, portraying the endocardial border outside the epicardium. CRF-CNN by contrast retains the endocardial border within the epicardium, as seen in the ground truth. In Table~\ref{tb:numb}, we report validation set Dice metrics for ED and ES time frames, and show that our DNLS method outperforms the other two methods for all the anatomical structures, particularly the myocardium. CNN is the fastest method as it was deployed with GPU, and DNLS is the most computationally expensive method due to its complex optimisation process.






==> sections/results_.tex <==
% !TeX root=../paper.tex

%\section{Experimental results}
%\label{sec:experiments}
%\textbf{Data:} Experiments were performed using short-axis CMR images from 430 PH patients. For each patient 10 to 16 short-axis slices were acquired roughly covering the whole heart. Each short-axis image has resolution of $1.5 \times 1.5 \times 8.0\;\rm{mm}^3$. Due to the large slice thickness of the short-axis slices and the inter-slice shift caused by respiratory motion, we train the FCN in a 2D fashion and apply the DNLS method to segment each slice separately. The ground truth region labels were generated using a semi-automatic process which included a manual correction step by an experienced clinical expert. Region labels for each subject contain the left and right ventricular blood pools and myocardial walls for all 430 subjects at end-diastolic (ED) and end-systolic (ES) frames. The ground truth edge labels are derived from the region label maps by identifying pixels with label transitions. The dataset was randomly split into training datasets (400 subjects) and validation datasets (30 subjects). For image pre-processing, all training images were reshaped to the same size of $160 \times 160$ with zero-padding, and image intensity was normalised to the range of $[0, 1]$ before training. 
%
% \textbf{Parameters:} The following parameters were used for the experiments in this work: First, there are six parameters associated with finding a desirable solution to (\ref{eq:transformedFunction}). They are the weighting parameter $\lambda$ (1), regularisation parameter $\epsilon$ (1.5), two levels $c_1$ (0) and $c_2$ (8), time step $t$ (0.1), and iteration number (200). Second, for training the network, we use Adam SGD with learning rate (0.001) and batch size (two subjects) for each of 50000 iterations. The weight $\alpha$ in (\ref{eq:REloss}) is set to 1. We perform data augmentation on-the-fly, which includes random translation, rotation, scaling and intensity rescaling of the input images and labels at each iteration. In this way, the network is robust against new images as it has seen millions of different inputs by the end of training. Note that data augmentation is crucial to obtain better results. Training took approx. 10 hours (50000 iterations) on a Nvidia Titan XP GPU, while testing took 5s in order to segment all the images for one subject at ED and ES. 
%\begin{figure}[h!] 
%\vspace{-10pt}
%\centering  
%{\includegraphics[width=0.99\textwidth]{figure/compare1.pdf}}\\
%\vspace{-5pt}
%\caption{Visual comparison of segmentation results from the vanilla CNN, CRF-CNN and proposed method. LV$\&$RV cavities and myocardium are delineated using yellow and red contours. GT stands for ground truth.}
%\label{fig:visual}
%\vspace{-20pt}
%\end{figure}

%\begin{table}[h!]
%\vspace{-20pt}
%\centering
%\caption{Quantitative comparison of segmentation results from the vanilla CNN, CRF-CNN and proposed method, in terms of Dice metric (mean$\pm$standard deviation) and computation time at testing stage.}
%\begin{tabular}{ccccc} \toprule
%{Methods} & {LV\&RV Cavities}     & {Myocardium} & {Time} \\ \midrule
%Vanilla CNN \cite{bai2017human}            & 0.902$\pm$0.047          & 0.703$\pm$0.091           & $\sim$\textbf{0.06}s  \\
%CRF-CNN     \cite{krahenbuhl2011efficient} & 0.911$\pm$0.045          & 0.712$\pm$0.082           & $\sim$2s  \\
%Proposed DNLS                              &\textbf{0.925$\pm$0.032} & \textbf{0.772$\pm$0.058}  & $\sim$5s  \\ \midrule
%\end{tabular}
%\label{tb:numb}
%\vspace{-15pt}
%\end{table}


\begin{table}[h!]
\centering
\caption{Quantitative comparison of segmentation results from the vanilla FCN, FCN-CRF and proposed method, in terms of Dice metric (mean$\pm$standard deviation) and computation time at testing stage.}
\vspace{3pt}
\begin{tabular}{ccccc} \toprule
{Methods} & {LV\&RV Cavities}     & {Myocardium} & {Time} \\ \midrule
Vanilla FCN             & 0.902$\pm$0.047          & 0.703$\pm$0.091           & $\sim$\textbf{0.06}s  \\
FCN-CRF      & 0.911$\pm$0.045          & 0.712$\pm$0.082           & $\sim$2s  \\
Proposed DNLS                              &\textbf{0.925$\pm$0.032} & \textbf{0.772$\pm$0.058}  & $\sim$5s  \\ \midrule
\end{tabular}
\label{tb:numb}

\end{table}

%\textbf{Comparsion:} The segmentation performance was evaluated by computing the Dice overlap metric between the automated and ground truth segmentations for LV $\&$ RV cavities and myocardium. We compared our method with the vanilla CNN proposed in \cite{bai2017human}, the code of which is publicly available. DNLS was also compared with the vanilla CNN with a conditional random field (CRF) \cite{krahenbuhl2011efficient} refinement (CRF-CNN). In Fig~\ref{fig:visual}, visual comparison suggests that DNLS provides significant segmentation improvements over CNN and CRF-CNN. For example, at the base of the right ventricle both CNN and CRF-CNN fail to retain the correct anatomical relationship between endocardium and epicardium portraying the endocardial border outside the epicardium. CRF-CNN by contrast retains the endocardial border within the epicardium, as described in the ground truth. In Table~\ref{tb:numb}, we report their Dice metric of ED and ES time frames in the validation dataset and show that our DNLS method outperforms the other two methods for all the anatomical structures, especially for the myocardium. CNN is the fastest method as it was deployed with GPU, and DNLS is the most computationally expensive method due to its complex optimisation processes. 





